In-Context Learning for Zero-Shot Speed Estimation of BLDC motors

Accurate speed estimation in sensorless brushless DC motors is essential for high-performance control and monitoring, yet conventional model-based approaches struggle with system nonlinearities and parameter uncertainties. In this work, we propose an in-context learning framework leveraging transformer-based models to perform zero-shot speed estimation using only electrical measurements. By training the filter offline on simulated motor trajectories, we enable real-time inference on unseen real motors without retraining, eliminating the need for explicit system identification while retaining adaptability to varying operating conditions. Experimental results demonstrate that our method outperforms traditional Kalman filter-based estimators, especially in low-speed regimes that are crucial during motor startup.

==> sections/experimental_results.tex <==
\section{Experimental results}

\subsection{Experimental setup}

\subsection{Simulator for the class of BLDC motors}

\subsection{Benchmark: Extended Kalman Filter}

\subsection{Experimental results}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/boxplot.pdf}
    \caption{Boxplot}
    \label{fig:boxplot}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/gridplot.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure*}

==> sections/experimental_results_RB.tex <==
\section{Experimental results}
\subsection{Experimental setup}
The experimental setup used to test this methodology is composed of:
%
\begin{itemize}
    \item[-] A BLDC motor (Maxon EC-i 40). It has a 7 pole pairs, a rated power of 100W, rated voltage of 48V and a rated speed of 4390rpm. It is equipped with a Hall sensor, which allows us to measure the rotor position and speed for testing. The motor is rigidly clamped to a vertical surface.
    \item[-] A bidirectional power supply, with a rated power of 6kW.
    \item[-] A three-phase motor controller: a demonstration board EVSPIN32G4 (STMicroelectronics) on which a FOC architecture is implemented.
    \item[-] A set of disks that can be mounted on the motor shaft as inertia loads. The disks' radii ($R_d$), masses ($M_d$) and inertia ($J_d$) can be found in Tab. \ref{tab:disk_specs}. Disk configuration $S^0$ was employed in the training phase, while the others were used for testing purposes.
    \item[-] An external computing unit: x64 based pc, 12th Gen Intel Core i7-12700H (4.70 GHz, 14 cores), 16Gb RAM, NVIDIA RTX 3070 Ti Laptop GPU (4Gb). It can communicate with the motor controller through a UART-based network ($f_s = 1$kHz), which allows us to set the gains for the FOC algorithms and the reference speed profiles, and to collect experimental data. Furthermore, this pc was used to develop and run the simulator presented in the next subsection, and to train the transformer model described above.
\end{itemize}
%
\begin{figure}[]
	\centering
	\includegraphics[width=0.8\linewidth, trim=0cm 11cm 0cm 6cm,clip]{figs/motore_disco.jpeg}\vspace{-.2cm}
	\caption{Experimental setup for a specific configuration. Note that, the motor and the inertial load are connected through a spindle.}
	\label{fig:setup}\vspace{-.3cm}
\end{figure}

% \begin{table}[tb]
% \centering
% \addtolength{\tabcolsep}{-6pt} 
% \begin{tabular}{lcccccc}
% \hline
%          & $S^0$       & $S^1$       & $S^2$       & $S^3$      & $S^4$       & $S^5$     \\ \hline 
% $r$              & 0.05        & 0.04        & 0.06        & 0.075      & 0.08        & 0.09      \\
% $m$               & 0.114       & 0.088       & 0.175       & 0.207      & 0.212       & 0.212     \\
% $J$ & $1.425\cdot10^{-4}$ & $7.041\cdot10^{-5}$ & $3.150\cdot10^{-4}$ & $5.822\cdot10^{-4}$ & $6.784\cdot10^{-4}$ & $8.856\cdot10^{-4}$\\
% \hline
% \end{tabular}
% \caption{Load disks configurations}
% \label{tab:disk_specs}
% \addtolength{\tabcolsep}{6pt} 
% \end{table}

\begin{table}[]
\centering
\caption{Load disks configurations}
\begin{tabular}{cccc}
\hline
 & $r$ [m]  &  $m$ [kg]  & $J$ [kg$\cdot m^2$]  \\
\hline
$S^0$ & 0.05  & 0.114 & $1.425\cdot10^{-4}$ \\
$S^1$ & 0.04  & 0.088 & $7.041\cdot10^{-5}$ \\      
$S^2$ & 0.06  & 0.175 & $3.150\cdot10^{-4}$ \\
$S^3$ & 0.075 & 0.207 & $5.822\cdot10^{-4}$ \\
$S^4$ & 0.08  & 0.212 & $6.784\cdot10^{-4}$ \\
$S^5$ & 0.09  & 0.212 & $8.856\cdot10^{-4}$ \\
\hline
\end{tabular}
\label{tab:disk_specs}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/OL_traj.pdf}
    \caption{Different configurations speed response when subject to the same quadrature current reference profile}
    \label{fig:OL}
\end{figure}

\subsection{Simulator for the class of BLDC motors}
\begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{figs/gridplot_5.pdf}
    \caption{Contextual filter (orange) and EKF (blue) estimations, from disk configuration $S^1$ (first column) to $S^5$ (last column). The last row highlight the average estimation error at a given time, and its standard deviation}
    \label{fig:gridplot}
\end{figure*}
The metadataset (\ref{eq:meta-set}) was generated through a BLDC motor simulator. The main idea behind this approach is that by perturbing the parameters of a digital twin, we can generate trajectories that are representative of the overall BLDC class $f = \mathcal{S}(\theta)$.
%
The simulator is composed of a BLDC motor, a three-phase inverter, and a FOC nested control loop, consisting in a PI speed controller, and two PI current controller for the direct and quadrature currents $i_d$ and $i_q$.
The parameters that the user is allowed to modify are $\theta=[R_s,L_s,\lambda_m,J_m,J_d,B_m,K_p,K_i]$, representing respectively the stator resistance and inductance, the maximum flux linkage, the motor inertia, the disk inertia, the viscous damping coefficient, the PI speed controller proportional and integral gains.
%
The motor and controller parameters were tuned to sufficiently match the open loop trajectories observed on the real motor, equipped with disk configuration $S^0$. Then, the following parameters were randomly perturbed before generating each trajectory in the metadataset:
% \begin{itemize}
%     \item The stator resistance $R_s$
%     \item The stator inductance $L_s$
%     \item The maximum flux linkage $\lambda_m$
%     \item The motor inertia $J_m$
%     \item The disk inertia $J_d$
%     \item The motor viscous damping coefficient $B_m$ 
%     \item The speed PI controller coefficient $K_p$ and $K_i$
% \end{itemize}
Each parameter $P_i$ but $J_d$ is perturbed by randomly extracting a value in the range $[P_n - 50\%, P_n + 50\%]$ with a uniform distribution, where $P_n$ is the nominal value obtained in the simulator tuning. The disk inertia is instead perturbed in a range $[I_{d,n}/10, I_{d,n}\times10]$, where $I_{d,n}$ is the nominal disk inertia, in order to cover the entirety of the studied disk configurations.
The number of pole pairs $p$ was kept constant at 7, as in the real motor.
%
The simulated trajectories consists in closed loop experiments with a speed profile structured as follows: 
\begin{equation}\label{eq:sim}
r(t) = \begin{cases}
0 &\text{if $t<0.5s$}\\
r_1 &\text{if $t\geq0.5s \ \wedge \ t<2.5s$}\\
r_2 &\text{if $t\geq2.5s \ \wedge \ t<4.5s$}\\
0 &\text{if $t\geq4.5s \ \wedge \ t<5s$}\\
\end{cases}
\end{equation}
Where $r(t)$ is the reference speed, and $r_1$ and $r_2$ are two random values extracted uniformly in the range $[0, 400]$ rpm. The maximum speed of 400 rpm was chosen in coherence with the sampling time $T_s = 0.01s$, for the reasons stated in subsection \ref{subsec:alias}.


\subsection{Testing dataset}\label{subsec:test_data}
A series of experimental data was collected on the real motor, to test the performances on the proposed filter. For each configuration, 15 randomized closed-loop speed profiles were observed. Each profile consists in a sequence of steps, whose amplitude and duration are randomly extracted in the ranges $[50, 400]$ rpm and $[3, 5]$ s respectively, for a total duration of 22s. furthermore, a fixed profile was chosen across each configuration, with the following structure:
\begin{equation}
r(t) = \begin{cases}
100 &\text{if $t<5s$}  \\
200 &\text{if $t\geq5s$}\ \wedge \ t<10s\\
300 &\text{if $t\geq10s$} \wedge \ t<15s\\
150 &\text{if $t\geq15s$} \wedge \ t<20s\\
\end{cases}
\end{equation}

\subsection{Benchmark: Extended Kalman Filter}
In order to assess the quality of our filter, a set of EKF was designed to provide a comparative benchmark. Each EKF is tuned on one of the disk configuration; for each, 5 additional randomized profile were collected, and used to design the EKF.
%
The same signals used for the contextual filters are passed to the EKF, which consequently uses as input the voltages $v_{\alpha}, v_{\beta}$, and outputs currents $i_{\alpha}, i_{\beta}$. The overall model uses as states the vector $[i_d, i_q, \omega, \theta_e]$:

\begin{equation}
\begin{cases}
\dot{i}_d = -\frac{R_s}{L_s} \ i_d + i_q \ \omega + \frac{\cos{\theta_e}}{L_s} \ v_\alpha + \frac{\sin{\theta_e}}{L_s} \ v_\beta + \eta_1\\
\dot{i}_q = -\frac{Rs}{Ls} \ i_q + (-i_d + \frac{\lambda_m}{L_s} ) \ \omega -  \frac{\sin{\theta_e}}{L_s} \ v_\alpha + \frac{\cos{\theta_e}}{L_s} \ v_\beta + \eta_2\\
\dot{\omega} = \frac{3}{2}\frac{p\ \lambda_m}{J_{tot}}\ i_q - \frac{B_m}{J_{tot}} \ \omega + \eta_3 \\
\dot{\theta}_e = p\ \omega + \eta_4 \\
i_\alpha = \cos{\theta_e}\ i_d - \sin{\theta_e}\ i_q + \xi_1\\
i_\beta = \sin{\theta_e}\ i_d - \cos{\theta_e}\ i_q + \xi_2 \\
i_{d,0} = \bar{i}_{d,0} + \zeta_1 \\
i_{q,0} = \bar{i}_{q,0} + \zeta_2 \\
\omega_{0} = \bar{\omega}_{0} + \zeta_3 \\
\theta_{e,0} = \bar{\theta}_{e,0} + \zeta_4
\end{cases}
\end{equation}
Where $J_{tot}= J_m + J_d$ represents the overall inertia, and $\eta = [\eta_1,\eta_2,\eta_3,\eta_4] \sim \mathcal{N}(0,Q)$, $\xi = [\xi_1,\xi_2] \sim \mathcal{N}(0,R)$, and $\zeta = [\zeta_1,\zeta_2,\zeta_3,\zeta_4] \sim \mathcal{N}(0,P_0)$ are white noises affecting the process, measurement, and initial state respectively. The model implicitly uses the Park transform to convert the inputs and outputs from the $\alpha \beta$ framework to the direct and quadrature one.
$R_s, L_s, \lambda_m, J_{tot}, \text{ and } B_m$ were obtained from the additional experiments. 
The covariance matrices $R$, $Q$, and $P_0$ used by the EKF are defined as:
\begin{align}
    R = \mathrm{diag}(1,1), \quad Q = \mathrm{diag}(q_1,q_2,q_3,q_4), \\
    \quad P_0 = \mathrm{diag}(10^{-6},10^{-6},10^{-6},p_0),
\end{align}
% \begin{equation}
% R = \begin{bmatrix}
% 1 & 0 \\
% 0 & 1 
% \end{bmatrix} \qquad
% Q = \begin{bmatrix}
% q_1 & 0 & 0 & 0 \\
% 0 & q_2 & 0 & 0 \\
% 0 & 0 & q_3 & 0 \\
% 0 & 0 & 0 & q_4 
% \end{bmatrix}    
% \end{equation}
%
% \begin{equation}
% P_0 = \begin{bmatrix}
% 10^{-6} & 0 & 0 & 0 \\
% 0 & 10^{-6} & 0 & 0 \\
% 0 & 0 & 10^{-6} & 0 \\
% 0 & 0 & 0 & p_0 
% \end{bmatrix}    
% \end{equation}
%
% Where $R$ is the covariance of the measurement noise, $Q$ is the covariance of the process noise, and $P_0$ is the initial state covariance.
% $q_1,q_2,q_3,q_4,\text{ and } p_0$ were chosen to minimize the estimation error of $\omega$. We use $x_0 = [0,0,0,0]$ as the initial state, and we assume that at the start of our experiment, the motor is still and no current is flowing, although the exact initial angle is unknown, hence the structure of $P_0$.
Where $q_1,q_2,q_3,q_4,\text{ and } p_0$ are tunable parameters, chosen to minimize the estimation error of $\omega$. We use $x_0 = [\bar{i}_{d,0},  \bar{i}_{q,0},  \bar{\omega}_{0}, \bar{\theta}_{e,0}] = [0,0,0,0]$ as the initial state; we assume that at the start of our experiment, the motor is still and no current is flowing; however, the exact initial angle is unknown, hence the structure of $P_0$.
Finally, the obtained EKF were applied to the other experiments with the respective disk configurations.

\subsection{Experimental results}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figs/multiplot_5.pdf}
    \caption{Average estimation along the fixed reference experiments}
    \label{fig:multiplot}
\end{figure}
%
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figs/boxplot_5.pdf}
    \caption{Estimation rmse across the disk configurations}
    \label{fig:boxplot}
\end{figure}
%
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/high_speed_plot_5.pdf}
    \caption{Experimental profiles at higher velocities, with disk configurations from $S^1$ (on the left) to $S^5$ (on the right).}
    \label{fig:high}
\end{figure*}
In Fig. \ref{fig:gridplot}, we can see the estimations of the contextual filter and the EKF; in the last row the average error across the 15 profiles at a given time is shown along with its standard deviation. Furthermore, in Fig. \ref{fig:multiplot} the average estimation across the 6 configurations for the fixed profile experiments, and its standard deviation are presented. It is clear how the contextual filter is more consistent in it estimations. This is corroborated by the comparison in estimation rmse for each disk configuration presented in Fig. \ref{fig:boxplot} highlighting how the contextual filter outperforms the EKF, in terms of average rmse and its variance, in all but one configuration, in whch they show similar results. One must also consider the fact that, for each configuration, model identification and parameter tuning from real-world data was required to design an appropriate EKF, while the contextual filter only required simulated data and needed no modification to work on a specific configuration.

\subsection{Beyond the aliasing}
As mentioned in section \ref{subsec:alias}, the choice of a sampling time $T_s>>T^{eval}$ can introduce an aliasing problem. While the recursive architecture of our filter is able to mitigate the issue, such is not the case for the EKF. To demonstrate the fact, a second filter was trained on simulated trajectories equivalent to the ones described in (\ref{eq:sim}), but in which the coefficients $r_1$ and $r_2$ are extracted in the range $[0,4000]$ rpm. Analogously, we collected data from the real motor by providing randomized speed profiles such as the ones described in section \ref{subsec:test_data}, but in which the step amplitude is extracted in the range $[250, 2500]$ rpm. An exemplificative profile for each disk configuration can be seen in Fig. \ref{fig:high}: the contextual filter can estimate the speed of the real motor correctly. On the other hand, it can be seen how the EKF can sometimes track the motor at lower speed, but fails to do so as the velocity increases.

==> sections/introduction.tex <==
\section{introduction}\label{sec:introduction}
Accurate speed estimation in sensorless brushless DC (BLDC) motors is crucial for achieving high-performance control and reliable monitoring. Traditional model-based estimation approaches, such as Kalman filters and observers \cite{kalman1960new, kandepu2008adaptive}, often struggle to handle the inherent nonlinearities and parameter uncertainties present in real-world motor systems. These limitations can significantly impact estimation accuracy, particularly in challenging operating conditions such as low-speed regimes during motor startup.

Recent advances in deep learning and transformer-based models \cite{vaswani2017attention, radford2019language} have demonstrated remarkable capabilities in various sequence modeling tasks, including system identification and control \cite{krishnan2016structured, bolz2023deep}. Inspired by these developments, we propose a novel in-context learning framework that leverages transformer-based architectures to perform zero-shot speed estimation in BLDC motors using only electrical measurements.

Unlike conventional techniques that require extensive system identification and parameter tuning \cite{chiang2021model, park2020data}, our approach trains a contextual filter offline on simulated motor trajectories. This allows real-time inference on unseen motor instances without the need for retraining or explicit system identification, thereby enhancing adaptability to varying operating conditions. The core idea is to exploit the transformer’s ability to learn and generalize from sequential data, capturing the underlying motor dynamics implicitly from a history of input-output measurements.

Our contributions can be summarized as follows:
\begin{itemize}
    \item We formulate the speed estimation problem as a sequence modeling task and introduce a transformer-based in-context learning framework tailored for BLDC motors.
    \item We demonstrate that our method generalizes to unseen motors without requiring parameter updates, leveraging learned representations of motor dynamics.
    \item We validate the proposed approach through extensive experiments, showing superior performance compared to Kalman filter-based estimators, especially in low-speed conditions where conventional methods often fail.
\end{itemize}

Experimental results confirm that our method outperforms traditional model-based estimators, reducing speed estimation errors and enhancing robustness across different motor instances. This work opens new possibilities for data-driven estimation techniques in electric motor applications, eliminating the need for cumbersome parameter tuning and improving real-time adaptability.






%Letteratura sensorless BLDC

%Letteratura ICL

%The contribution of this work is the validation of the method firstly presented in \cite{bus24} on a real experimental case study, where we leverage a black-box digital twin for a class of BLDC motors for the design of the contextual filter, which allow successfully for zero-shot speed estimation on real BLDCs examples.
